MegaWika: Millions of reports and their sources across 50 diverse languages

To foster the development of new models for collaborative AI-assisted report generation, we introduce MegaWika, consisting of 13 million Wikipedia articles in 50 diverse languages, along with their 71 million referenced source materials. We process this dataset for a myriad of applications, going beyond the initial Wikipedia citation extraction and web scraping of content, including translating non-English articles for cross-lingual applications and providing FrameNet parses for automated semantic analysis. MegaWika is the largest resource for sentence-level report generation and the only report generation dataset that is multilingual. We manually analyze the quality of this resource through a semantically stratified sample. Finally, we provide baseline results and trained models for crucial steps in automated report generation: cross-lingual question answering and citation retrieval.

==> 70-future-work.tex <==
\section{Future Work}
\label{sec:future}

\kenton{Why do we need this section? Could the most essential parts be part of the conclusion? Spending more space on this than sections 2, 5, and 6 seems like the wrong move.}
PAQ-generated questions are occasionally non-sensical, or grammatically malformed, or otherwise irrelevant to the extracted answer span. This phenomenon is reflected in the evaluation results above. Future work will focus on ways to improve the quality of generated questions, whether by improving answer selection, or directly improving the quality of the question generation model.

One approach to indirectly improving the quality of the \qa{} pairs is to first improve the quality of the machine translation system that transfers Wikipedia passages to English prior to question generation. Our initial dataset collection and processing effort emphasized a balance between quality and computational tractability, given the limited scale of the JHU/HLTCOE cluster and its high level of usage. The MT model we therefore used worked acceptably well for high-resource languages like Spanish, but for very low-resource languages (e.g., Xhosa, Irish Gaelic, Khmer, etc.), translation quality suffered, sometimes enough that it doomed subsequent processing phases -- particularly answer selection and question generation. As a result, we recently embarked on a retranslation effort using Google Translate, intended ultimately to embrace the entire dataset. The improvement in quality is marked:
\begin{itemize}
    \item \textbf{Xhosa original}: UMzantsi Afrika, ngokusesikweni ubizwa ngokuba yirhiphabhlikhi yaseMzantsi Afrika (RSA), lilizwe elibuthume kwincakami yeAfrika.
    \item \textbf{M2M100}: South Africa, which is known as the South African Library (RSA), is a famous city in the southern part of Africa.
    \item \textbf{Google Translate API}: South Africa, officially called the Republic of South Africa (RSA), is a country on the tip of Africa.
\end{itemize}
The price paid for this approach, however, is that it is significantly slower.

Related to the issue of \qa{} pair quality is the desire to ensuring that the generated questions are answerable based on the cited source document\,---\,or in other words, encouraging the generation of questions that align or link the Wikipedia passage with the cited source document, by enforcing that the information asked about in the question must be present in both.

Finally, recall that \qa{} pairs are generated on the basis of the English-translated Wikipedia passage; then exact string match is used to locate the corresponding answer in the source document. But exact string match is only an expedient heuristic; it cannot find an answer span in the case that the answer is paraphrased, or in the case that the information required to answer the question is indeed present in the source, but is broken up across the document. Future work will focus on better methods for aligning the passage/source documents.

